SoftVQ-VAE: Efficient 1-Dimensional Continuous Tokenizer

Efficient image tokenization with high compression ratios remains a critical challenge for training generative models. We present SoftVQ-VAE, a continuous image tokenizer that leverages soft categorical posteriors to aggregate multiple codewords into each latent token, substantially increasing the representation capacity of the latent space. When applied to Transformer-based architectures, our approach compresses 256x256 and 512x512 images using as few as 32 or 64 1-dimensional tokens. Not only does SoftVQ-VAE show consistent and high-quality reconstruction, more importantly, it also achieves state-of-the-art and significantly faster image generation results across different denoising-based generative models. Remarkably, SoftVQ-VAE improves inference throughput by up to 18x for generating 256x256 images and 55x for 512x512 images while achieving competitive FID scores of 1.78 and 2.21 for SiT-XL. It also improves the training efficiency of the generative models by reducing the number of training iterations by 2.3x while maintaining comparable performance. With its fully-differentiable design and semantic-rich latent space, our experiment demonstrates that SoftVQ-VAE achieves efficient tokenization without compromising generation quality, paving the way for more efficient generative models. Code and model are released.

==> sec/1_main.tex <==


\begin{figure*}[th!]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/teaser.pdf}
    \vspace{-0.1in}
    \caption{ImageNet-1K 256$\times$256 and 512$\times$512 generation results of generative models trained on \softvq with 32 and 64 tokens. 
    % \xl{maybe change the row2-col1 image, too close to row1-col1 train}
    }
    \label{fig:teaser}
    \vspace{-0.2in}
\end{figure*}


\section{Introduction}
\label{sec:intro}



% generative modelling
\textit{Denoising}-based generative modeling has witnessed remarkable progress with recent advances, such as Diffusion Transformers (DiT) \cite{peebles2023scalablediffusionmodelstransformers}, Scalable Interpolant Transformers (SiT) \cite{ma2024sit}, and Masked Auto-Regressive models with diffusion loss (MAR) \cite{li2024autoregressiveimagegenerationvector}, to name a few. Denosing-based generative modeling not only presents impressive generation results on a wide range of modality, including natural language \cite{gong2022diffuseq,zheng2023reparameterized}, images \cite{ramesh2021zero,dhariwal2021diffusionmodelsbeatgans,rombach2022highresolutionimagesynthesislatent,lu2024simplifying,fan2024fluid}, videos \cite{ho2022video,blattmann2023stable,bar2024lumiere}, and audios \cite{popov2021grad,evans2024fast}, but also shows potential to unify the understanding and generation capabilities across modalities in multi-modal language models \cite{zhou2024transfusion,xie2024show,wang2024emu3,wu2024vila}. 


% image generation, discrete and continuous
% image tokenizers, VQ for discrete and KL for continuous
A core component of denoising-based generative models is the tokenizer \cite{kingma2013auto,higgins2017beta,van2017neural,razavi2019generating,esser2021taming,zeghidour2021soundstream,lee2022autoregressiveimagegenerationusing,yu2023language}, which compresses the raw data of each modality into a set of 
%\textit{continuous-valued}
latent tokens in either a \textit{discrete} or \textit{continuous} latent space.
% by training auto-encoder architectures with a reconstruction objective.
The compact latent space therefore allows for more efficient and better generative modeling \cite{rombach2022highresolutionimagesynthesislatent}. 
Among previous efforts, Kullback–Leibler Variational Auto-Encoders (\kl) \cite{kingma2013auto} and Vector Quantized Variational Auto-Encoders (\vq) \cite{van2017neural,razavi2019generating,esser2021taming} stand out as representatives of tokenizers which introduce continuous and discrete latent spaces, respectively.
The former constrains the latent space with a Gaussian distribution using \textit{re-parametrization} \cite{kingma2013auto} trick, and the latter makes its latent space a categorical discrete distribution with a codebook of finite vocabulary which requires \textit{straight-through} estimation \cite{bengio2013estimating}.

% \ch{problems of KL-VAE and VQ-VAE: (1) token length; (2) latent space }
% \ch{need to talk about KL-VAE is gaussian and VQ-VAE is lossy}
% problems: token length of reconstruction, token length of generation, latent space for diffusion models



% \begin{figure}[t!]
%     \centering
%     \hfill
%     \begin{subfigure}{0.49\linewidth}
%     \centering
%         \includegraphics[width=\linewidth]{example-image}
%         \caption{rFID vs \# Token}
%         \label{fig:rfid_token_model}
%     \end{subfigure}%
%     \hfill
%     \begin{subfigure}{0.49\linewidth}
%     \centering
%         \includegraphics[width=\linewidth]{example-image}
%         \caption{gFID vs \# Token}
%         \label{fig:gfid_token_model}
%     \end{subfigure}%
%     \hfill
%     \vspace{-0.1in}
%     \caption{Trade-off}
%     \label{fig:trade-off}
% \vspace{-0.2in}
% \end{figure}



Although both \kl and \vq (and their variants) have been predominantly adopted in many generative models \cite{rombach2022highresolutionimagesynthesislatent,peebles2023scalablediffusionmodelstransformers,chang2022maskgitmaskedgenerativeimage,sun2024autoregressive,zhou2024transfusion}, they still present two major challenges restricting the efficiency and effectiveness of generative modeling: (1) \textbf{the difficulty of achieving a higher compression ratio} \cite{chen2016variational} and 
% \textbf{the lack of semantics in their latent space}. 
(2) \textbf{the worse discriminative representations in their latent space than other self-supervised methods} \cite{he2022masked,chen2024deconstructing,yu2024representation,wu2024vila}.
% ,which restrict the efficiency and effectiveness of the downstream generative modeling, respectively.
% The efficiency of the downstream generative modeling is directly restricted by the compression ratio, especially for Transformer architectures \cite{vaswani2023attentionneed} with complexity quadratic to the number of latent tokens.
% Taking image tokenizer \cite{esser2021taming,rombach2022highresolutionimagesynthesislatent,stabilityai2023} as an example, it commonly compresses a raw image of resolution 256$\times$256 to 256 latent tokens and 512$\times$512 to 1024 tokens \cite{esser2021taming,rombach2022high}, which significantly limits the training and inference efficiency of generative models \cite{peebles2023scalablediffusionmodelstransformers,ma2024sit,li2024autoregressiveimagegenerationvector}.
% token length
% The efficiency of generative modeling is directly restricted by the compression ratio, especially for Transformer \cite{vaswani2023attentionneed} architectures with complexity quadratic to the number of latent tokens. 
The efficiency of downstream generative models, particularly Transformer-based architectures \cite{vaswani2023attentionneed}, is fundamentally constrained by their quadratic complexity to the number of latent tokens. Current image tokenizers \cite{esser2021taming,rombach2022highresolutionimagesynthesislatent,stabilityai2023} typically compress 256$\times$256 images to at least 256 tokens and 512$\times$512 images to at least 1024 tokens, creating a significant computational bottleneck for both training and inference of generative models \cite{peebles2023scalablediffusionmodelstransformers,ma2024sit,li2024autoregressiveimagegenerationvector}.
Many efforts have been made to reduce the number of latent tokens on the generative model side, such as merging \cite{peebles2023scalablediffusionmodelstransformers,ma2024sit,li2024imagefolder}, pooling \cite{li2023blip,song2024less,li2024tokenpacker}, and others \cite{luo2024feast,li2024mini,chen2024image}.
More studies have recently emerged to fundamentally reduce the token number of the tokenizer \cite{ge2023plantingseedvisionlarge,yu2024an,li2024imagefolder,chen2024deep}.
% more recent studies attempted to reduce the token number from the tokenizer using various techniques \cite{ge2023plantingseedvisionlarge,yu2024an,li2024imagefolder,chen2024deep}. 
For example, TiTok \cite{yu2024an} uses 128 tokens, achieving generation results comparable to 256 tokens by adding one extra decoder.
DC-AE \cite{chen2024deep} compresses the initial 1024 tokens of 512$\times$512 with 256 tokens.
% excels at the generation of 512$\times$512 images using 256 tokens, compared to 1024 tokens \cite{peebles2023scalablediffusionmodelstransformers}.
However, further increasing the compression ratio results in a significant degradation in the quality of reconstruction and therefore the generation \cite{chen2024deep}. 
% , as shown in \cref{fig:trade-off}. 

% However, a high compression ratio 
% A high compression ratio not only lead to \ch{summary challenges of high compression ratio} As shown in \cref{fig:trade-off}, \ch{talk about the trade-off}.
% \ch{Problem of high compression ratio of Kl and VQ}

% \ch{need to talk about continuous latent space is better than discrete latent space}

% semantics in latent space


% The representation quality of the latent space from the tokenizer has been shown to be essential for
% (multi-modal) 
% generative models to learn well both understanding \cite{ge2023making,wu2024vila} and generation \cite{ge2023plantingseedvisionlarge,lin2023sphinx,yu2024representation,li2024imagefolder}.
Beyond the compression challenge, the quality of the learned representations of the tokenizer poses another critical limitation.
While latent representations are crucial for both understanding \cite{ge2023making,wu2024vila} and generation tasks \cite{ge2023plantingseedvisionlarge,lin2023sphinx,yu2024representation,li2024imagefolder}, current tokenizers usually struggle to capture more discriminative features.
Earlier methods attempted to advance the training objectives and recipe to improve the latent space of the tokenizer \cite{esser2021taming,dong2023peco,gu2023rethinkingobjectivesvectorquantizedtokenizers,zhu2024scaling,chen2024deconstructing}.
Recently, \cite{ge2023plantingseedvisionlarge,zhang2024codebook,yu2024spae,zhu2024scaling,wu2024vila,li2024imagefolder,yu2024representation} has also explored the representation alignment of latent tokens.
However, due to the lossy nature \cite{shannon1949communication,nyquist1928certain} of the smoothness constraints in \kl and the discrete quantization in \vq \cite{higgins2017beta,chen2016variational,zhu2024addressing,fifty2024restructuring}, current tokenizers usually fall short in learning the semantics of the latent space \cite{wu2024vila}.
% \wjd{Can we call the second challenge misalignment?}
% \wjd{I'm new to the compression ratio, but would say the should will have some threshold according to information theory? What is the threshold and do current methods approach it?}

% \ch{Problem of injecting semantics into latent space of tokenizer}

% our method: two variants softvq-vae and gmm-vae
% converting VQ-VAE into a continuous tokenizer 
To address the aforementioned challenges, we present \textbf{\softvq}, a simple modification to \vq that converts it from a discrete tokenizer into a continuous one with a high compression ratio and a semantic-rich latent space. 
Specifically, we propose using a \textbf{soft} categorical posterior in VAE with a learnable codebook. 
This straightforward modification introduces a crucial capability: instead of the conventional one-to-one mapping between tokens and codewords in \vq, our approach enables the adaptive aggregation of multiple codewords into each latent token, substantially increasing the representation capacity of the latent space.
% Specifically, we propose using a \textbf{soft} categorical posterior in VAE with a learnable codebook, which allows the aggregation of multiple codewords into one latent token, in contrast to selecting a single codeword as one latent token in \vq. \wjd{To me it seems not hard to do it... How can we justify the idea?}
% With a Transformer auto-encoder architecture \cite{yu2021vector,ge2023plantingseedvisionlarge,li2023blip,yu2024an,li2024imagefolder}, \softvq thus uses much less number of 1-dimensional latent tokens, \ie, \textbf{32} and \textbf{64}, for both the reconstruction and subsequent generation tasks, without hurting the performance. 
We apply \softvq to the Transformer auto-encoder architecture \cite{yu2021vector,ge2023plantingseedvisionlarge,li2023blip,yu2024an,li2024imagefolder}, and we succeed in using much fewer 1-dimensional latent tokens (\ie, \textbf{32} and \textbf{64}) for both the reconstruction and subsequent generation tasks.
% without harming the performance.
% Since \softvq is now fully-differentiable, it does not require additional codebook loss or commit loss to learn the codebook. 
%Since \softvq is now fully-differentiable, its codebook can be directly learned without the codebook loss or commit loss as in \vq \cite{van2017neural,esser2021taming}. 
Since \softvq is now fully differentiable, it not only simplifies the learning of the codebook, not requiring the codebook loss or commit loss as in \vq \cite{van2017neural,esser2021taming}, but also enables better representation learning through direct alignment with pre-trained semantic features using a simple cosine similarity objective. 
% Theoretically, 
Our approach generalizes the K-Means \cite{lloyd1982least} latent space of \vq to Soft K-Means~\cite{dunn1973fuzzy} and further to Gaussian Mixture Models (GMM) \cite{reynolds2009gaussian}, while maintaining compatibility with existing \vq techniques \cite{jegou2010product,yu2023language,lee2022autoregressive,li2024imagefolder}.
We comprehensively demonstrate the efficiency and effectiveness of the proposed \softvq in image reconstruction and generation tasks, and show that:
% Our findings and contributions can be summarized as follows:
\begin{itemize}[leftmargin=1em,nosep]
\setlength\itemsep{0em}
    \item \softvq presents more consistent, robust, and high-quality reconstruction and generation results with various latent token lengths ranging from 256 to 32. 
    \item \softvq allows \textit{diffusion-based} DiT \cite{mentzer2023finite}, \textit{flow-based} SiT \cite{ma2024sit}, and \textit{autoregressive-based} MAR \cite{li2024autoregressiveimagegenerationvector} to achieve state-of-the-art generation results with only 64 and 32 tokens on both the 256$\times$256, with an FID of \textbf{1.78}, and 512$\times$512 on ImageNet benchmark, with an FID of \textbf{2.21}.
   \item  \softvq improves the inference throughput by \textbf{18}x and \textbf{10}x with 32 and 64 tokens to generate 256$\times$256 images, and \textbf{55}x with 64 tokens for generating 512$\times$512 images, with significantly lower GFLOPs for all models. 
   \item \softvq presents a more discriminative latent space through representation alignment. It also facilitates training efficiency by significantly improving training throughput and reduces training iterations by \textbf{2.3}x. 
\end{itemize}


% We further show that semantical latent space can be more easily and better learned by aligning the latent code with pre-trained semantic features using a simple cosine similarity objective. 
% Theoretically, the latent space of \softvq can be interpreted as performing Soft K-Means on the codewords~\cite{dunn1973fuzzy}, and we show that it can be further extended to a Gaussian Mixutre Model (GMM) \cite{reynolds2009gaussian} latent space, resulting in GMMVQ-VAE, compared to the K-Means \cite{lloyd1982least} latent space in \vq. 
% With the learnable codebook maintained as prototype and Gaussian means, respectively, previous techniques applicable to \vq \cite{jegou2010product,yu2023language,lee2022autoregressive,li2024imagefolder} are also compatible with \softvq.

% More importantly,  
% mention feature alignment

% results and contribution
% We comprehensively demonstrate the efficiency and effectiveness of the proposed \softvq in image generation tasks.
% We show that \softvq allows \textit{diffusion-based} DiT \cite{mentzer2023finite}, \textit{flow-based} SiT \cite{ma2024sit}, and \textit{autoregressive-based} MAR \cite{li2024autoregressiveimagegenerationvector} to achieve state-of-the-art generation results with only 64 and 32 tokens on both 256$\times$256 and 512$\times$512 ImageNet benchmark.
% \ch{Add FID results}
% Moreover, \softvq improves the inference throughput by \textbf{18}x with 32 tokens and \textbf{10}x with 64 tokens for generating 256$\times$256 images, and \textbf{100}x with 32 tokens and \textbf{55}x with 64 tokens for 512$\times$512 images. 


% , and reduces training time by 
% \ch{mention semantics?}


% \ch{Add results and contribution here}.
% Our contribution can be summarized as follows. 
% \begin{itemize}[leftmargin=1em,nosep]
% \setlength\itemsep{0em}
%     \item softvq
%     \item 64 tokens sota; 32 tokens beat w/o REPA
% \end{itemize}




\section{Preliminary}
\label{sec:prelimiary}

We present an overview of the tokenizers, \ie, \kl \cite{kingma2013auto} and \vq \cite{van2017neural}, and denoising-based generative models, \ie, DiT \cite{peebles2023scalablediffusionmodelstransformers}, SiT \cite{ma2024sit}, and MAR \cite{li2024autoregressiveimagegenerationvector}, in this section.
% , which will be used throughout this paper.
% \ch{need to fix some notation}


\subsection{Image Tokenizer}

The architecture of image tokenizer generally resembles auto-encoders, consisting of two main components: an encoder $\mathcal{E}$ and a decoder $\mathcal{D}$, parameterized by $\phi$ and $\theta$, respectively.
Given an input image $\mathbf{x} \in \mathbb{R}^{H \times W \times 3}$, the encoder $\mathcal{E}$ maps the high-dimensional $\mathbf{x}$ to a lower-dimensional latent representation $\mathbf{z} = \mathcal{E}(\mathbf{x};\phi)$.
The latent representations can have varying shapes depending on the encoder architecture. 
% such as 3-dimensional outputs from CNNs and 2-dimensional outputs from Transformers. 
We generally view the latent representation as a set of latent tokens $\mathbf{z} = [\mathbf{z}^{[0]}, \mathbf{z}^{[1]}, \dots, \mathbf{z}^{[L]}] \in \mathbb{R}^{L \times D}$, where $L$ is the number of tokens and $D$ is the dimension of the latent representation.
For basic auto-encoders (AE), the decoder takes latent tokens as input and reconstructs the original signal $\hat{\mathbf{x}} = \mathcal{D}(\mathbf{z};\theta)$ by minimizing the reconstruction loss with $\mathbf{x}$.
% Usually a perceptual (LPIPS) loss \cite{larsen2016autoencoding,johnson2016perceptual,dosovitskiy2016generating,zhang2018unreasonableeffectivenessdeepfeatures} and an adversarial (GAN) loss \cite{goodfellow2020generative,isola2018imagetoimagetranslationconditionaladversarial} are optimized jointly with the reconstruction loss for better perceptual quality and higher compression rate \cite{esser2021taming}.


Variational auto-encoders (VAE) \cite{kingma2013auto} extend the basic AE by introducing a probabilistic perspective on the latent space. 
Specifically, VAE approximates a posterior distribution $p(\mathbf{z} | \mathbf{x})$ with a learned distribution $q_{\phi}(\mathbf{z}|\mathbf{x})$ from the encoder, assuming that $\mathbf{x}$ is generated by the unobserved latent $\mathbf{z}$ with a prior distribution $p(\mathbf{z})$. 
The decoder instead takes a set of sampled latent tokens $\mathbf{z} \sim q_{\phi}(\mathbf{z}|\mathbf{x})$ from the posterior and aims to learn the marginal likelihood of data in a generative process by optimizing the evidence lower bound (ELBO):
$\max_{\phi, \theta} \mathbb{E}_{q_{\phi}(\mathbf{z} | \mathbf{x})} \log p_{\theta}(\mathbf{x} | \mathbf{z}) - \mathcal{L}_{\mathrm{kl}}(  q_{\phi} (\mathbf{z} | \mathbf{x}) | p(\mathbf{z}) ) $. 
To make the optimization tractable, assumptions have been made on the prior, leading to different variants of VAE. 

%$ \noindent \textbf{KL-VAE}. 
\noindent \textbf{KL-VAE} \cite{kingma2013auto,higgins2017beta} parametrizes both the prior and posterior as Gaussians.
The prior $p(\mathbf{z})$ is assumed to be the isotropic unit Gaussian $\mathcal{N}(0, 1)$. 
The \textit{continuous} latent code is parameterized with posterior mean $\boldsymbol{\mu}_{\phi}$ and variance $\boldsymbol{\sigma}^2_{\phi}$ predicted by the encoder using the ``re-parametrization" trick with a noise variable $\boldsymbol{\varepsilon}$ from standard Gaussian:
\begin{equation}
\resizebox{.8\linewidth}{!}{$
\begin{split}
    & \textit{posterior:  } q_{\phi}(\mathbf{z} | \mathbf{x}) = \mathcal{N}(\mathbf{z}; \boldsymbol{\mu}_{\phi}(\mathbf{x}), \boldsymbol{\sigma}^2_{\phi}(\mathbf{x})) \\
    & \textit{latent:  } \mathbf{z} = \boldsymbol{\mu}_{\phi}(\mathbf{x}) + \boldsymbol{\sigma}_{\phi}(\mathbf{x}) \odot \mathbf{\varepsilon}, \quad \epsilon \sim \mathcal{N}(0, \mathbf{I}) \\
    & \textit{kl: } \mathcal{L}_{\mathrm{kl}} = -\frac{1}{2}\left(1+\log \left(\boldsymbol{\sigma}_{\phi}^2(\mathbf{x})\right)-\boldsymbol{\mu}_{\phi}(\mathbf{x})^2-\boldsymbol{\sigma}_{\phi}^2(\mathbf{x})\right)
\end{split}
$}
\label{eq:kl}
\end{equation}
While KL-VAE is widely used in diffusion models, it is known to have the ``posterior-collapse" issue \cite{chen2016variational}. 
In addition, the KL loss weight usually imposes a trade-off between the quality of reconstruction and the smoothness of its latent space \cite{tschannen2025givt}, preventing high compression ratio and the learning of semantics in the latent space of \kl. 


% \noindent \textbf{VQ-VAE}. 
\noindent \textbf{VQ-VAE} \cite{van2017neural,esser2021taming}, in contrast, generates latent code in a \textit{discrete} space by taking the posterior as a $K$-way deterministic categorical distribution against a learnable codebook $\mathcal{C} = [\mathbf{c}^{[0]}, \dots, \mathbf{c}^{[K]}] \in \mathbb{R}^{K \times D}$, with $\mathbf{c}$ as the codeword:
\begin{equation}
\resizebox{.9\linewidth}{!}{$
\begin{split}
  & \textit{posterior: } q_{\phi}(\mathbf{z} = k | \mathbf{x}) = 
   \begin{cases} 
      1 & \text{if } k = \argmin_{j} \| \hat{\mathbf{z}} - \mathbf{c}^{[j]} \|_2 \\
      0 & \text{otherwise} 
   \end{cases} \\
  & \textit{latent: } \mathbf{z} = \mathbf{c}^{[k]}, \quad \text{where } k = \argmin_{j} \| \hat{\mathbf{z}} - \mathbf{c}^{[j]} \|_2  \\ 
  & \textit{kl: } \mathcal{L}_{\mathrm{kl}} = \log K  \\
\end{split}
$}
\label{eq:vq}
\end{equation}
Due to the non-differentiable $\argmin$, a ``straight-through'' trick \cite{bengio2013estimating} is adopted to approximate the gradient of the encoder output $\hat{\mathbf{z}}$ by directly copying gradient from the decoder input $\mathbf{z}$. 
% Due to the ''straight-through'' estimation, 
Since the reconstruction objective does not impose direct gradients on the codebook $\mathcal{C}$, VQ-VAE additionally uses a codebook loss as $\|\text{sg}[\hat{\mathbf{z}}] - \mathbf{c}\|_2$ to move codewords toward the encoder output, along with a commit loss $\|\hat{\mathbf{z}} - \text{sg}[\mathbf{c}]\|_2$ to prevent arbitrary growth of codewords, where $\text{sg}[\cdot]$ denotes stop-gradient.
The broken gradient hinders high compression ratio and latent space learning \cite{huh2023straightening,fifty2024restructuring}.
% of \vq \cite{huh2023straightening,fifty2024restructuring}. 

% \ch{Needs to talk more about the limitation of VQ-VAE}

% codebook loss, commit loss, straight through 


\subsection{Denoising-based Generative Models}

Denoising-based generative models synthesize images by progressively transforming Gaussian noise $\boldsymbol{\varepsilon} \sim \mathcal{N}(0, \mathbf{I})$ into tokenizer latent codes $\mathbf{z}$ through a forward process \cite{sohl2015deep,ho2020denoising}:
\begin{equation}
\mathbf{z}_t = \alpha_t \mathbf{z} + \sigma_t \varepsilon,
\label{eq:forward}
\end{equation}
where $\alpha_t$ and $\sigma_t$ are a decreasing and increasing function of $t$, and $t \in [0, T]$ \cite{kingma2024understanding}. In this paper, we adopt three approaches to implementing this denoising process as follows.
% in this paper.


% \noindent \textbf{DiT}.
\noindent \textbf{DiT} \cite{peebles2023scalablediffusionmodelstransformers} is a diffusion-based model with a transformer architecture. 
It formulates the process through a forward-time stochastic differential equation (SDE), where $\mathbf{z}_t$ converges to $\mathcal{N}(0, \mathbf{I})$ as $t \rightarrow T$. 
Generation occurs via a reverse-time SDE \cite{anderson1982reverse}, with the model trained to predict noise $\boldsymbol{\varepsilon}$ at randomly sampled timesteps. 
Due to the long token length of the tokenizer \cite{stabilityai2023} used in DiT, it has several variants to merge tokens at the input of the transformer backbone.

% It learns the reverse process. 


% \noindent \textbf{SiT}

\noindent \textbf{SiT} \cite{ma2024sit} instead uses stochastic interpolants \cite{albergo2023stochastic} and performs denoising via probability flow ordinary differential equation (PF ODE). 
The model learns the ODE's velocity field \cite{lipman2022flow} by minimizing mean-squared-error (MSE) with the interpolated noise.
This velocity field defines a score function for sample generation, analogous to DiT's reverse-time SDE.



% \noindent \textbf{MAR}

\noindent \textbf{MAR} \cite{li2024autoregressiveimagegenerationvector} 
combines diffusion with autoregressive generation. 
Unlike DiT and SiT's parallel denoising of all latent tokens, MAR adopts an encoder-decoder transformer architecture \cite{he2022masked} that progressively denoises tokens in a ``next-set'' autoregressive manner \cite{tian2024visualautoregressivemodelingscalable}, starting from masked tokens, similar to MaskGIT \cite{chang2022maskgitmaskedgenerativeimage} and MAGE \cite{li2023magemaskedgenerativeencoder}.
% extends diffusion-based denoising into auto-regressive models. 
% It combines an encoder-decoder transformer architecture and masked generative models \cite{chang2022maskgitmaskedgenerativeimage,li2023magemaskedgenerativeencoder}, with diffusion loss.
% Instead of denoising all latent tokens in parallel as in DiT and SiT, MAR progressively performs denoising based on previously denoised tokens in next-set auto-regressive fashion, starting from the masked tokens. 

% Each of these models operates under the framework of denoising-based generation, progressively refining initial noisy or partial inputs through well-defined mathematical processes. These models will be used in our experiments to evaluate and compare their performance across different image synthesis tasks.





\section{Method}
\label{sec:method}

In this section, we present \softvq, a novel 1D continuous tokenizer with a high compression ratio and a semantic-rich latent space. 
We first introduce the architecture and the formulation of \softvq. 
Then, we show that \softvq can learn semantics easily by aligning its latent tokens with pre-trained features via its fully-differentiable property.
% / and is compatible with previous techniques of improving \vq. 

% In this section, we introduce the architecture and posterior of \softvq. 

% \ch{overview: transformer with learnable code for 1D latent codes, soft-vq for aggregating multiple codewords in one latent code which reducing the token length while maintain reconstruction quality, representation alignment for better latent space thanks to the fully-differentiable soft-vq}

\subsection{Architecture}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.98\linewidth]{figures/pipeline.pdf}
    \vspace{-0.1in}
    \caption{Illustration of \softvq. Left: Transformer encoder-decoder architecture with image tokens, arbitrary length of latent tokens, and mask tokens. Right top: fully-differentiable SoftVQ illustration. Right bottom: latent space representation alignment.}
    \label{fig:architecture}
\vspace{-0.2in}
\end{figure}


We leverage Vision Transformer (ViT) \cite{dosovitskiy2021imageworth16x16words,yu2021vector} as the architecture for the encoder $\mathcal{E}$ and decoder $\mathcal{D}$ of \softvq.
Similarly to \citet{yu2024an}, instead of using the image features as latent, we initialize a set of extra 1D learnable tokens and use these tokens for reconstruction and subsequent generation.
With the self-attention mechanism, it allows the learnable tokens to adaptively aggregate different image tokens to obtain the latent tokens of SoftVQ, detailed in \cref{sec:method-softvq}. 
Specifically, for the encoder transformer with a patch size of $P$, an image $\mathbf{x} \in \mathbb{R}^{H \times W \times 3}$ is patchified into a sequence of image tokens $\mathbf{x}_p \in \mathbb{R}^{N \times D}$, where $N = \ HW / P^2$ and $D$ represent the token dimension size.
We then concatenate a set of learnable tokens $\mathbf{z}_l \in \mathbb{R}^{L \times D}$ of length $L$ along with the image tokens as the input to the encoder, and retain only the output corresponding to the learnable latent tokens as the output of our encoder: $\hat{\mathbf{z}} = \mathcal{E}([\mathbf{x}_p; \mathbf{z}_l];\phi)$. 
% The latent tokens $\mathbf{z}$ are from SoftVQ

For the decoder, we reconstruct images from a sequence of learnable mask tokens $\mathbf{m} \in \mathbb{R}^{N \times D}$ \cite{bao2021beit,he2022masked}, concatenated with latent tokens: $\hat{\mathbf{x}} = \mathcal{D}([\mathbf{m};\mathbf{z}];\theta)$. 
We use a linear layer at the end of the decoder to regress the pixel values from the mask tokens.
For the image tokens at the encoder input and mask tokens at the decoder input, we apply 2D absolute position embeddings and 1D absolute position embedding for the latent tokens. 
Adopting more advanced position embedding techniques, such as RoPE \cite{su2024roformer,heo2025rotary}, may lead to better results and is left for future work. 
This design allows \softvq to use latent codes of arbitrary length, each adaptively associated with image tokens, for reconstruction and subsequent generative modeling, and model images of various resolutions using the same length of latent codes.
An overview of the model architecture is shown in \cref{fig:architecture}.

% Despite simple, with \softvq as the latent space, this design allows us to use latent codes of arbitrary length and high compression ratio for reconstruction and the subsequent generative modeling, and model images of various resolutions using the same length of latent codes. 



\subsection{\softvq}
\label{sec:method-softvq}

As discussed above, the high compression ratio of both KL-VAE and VQ-VAE usually results in a significant degradation of quality in reconstruction and latent space.
To overcome these limitations, we propose \softvq, a simple modification to VQ-VAE, which maintains the advantages of learning codewords to capture the data distribution while bridging it with more representation capacity as a continuous tokenizer. 
The core idea of \softvq is to allow each latent code to adaptively aggregate multiple codewords from the learnable codebook. 
Consequently, it imposes a \textit{soft} categorical distribution on the posterior from the encoder:
\begin{equation}
\resizebox{.75\linewidth}{!}{$
\begin{split}
    & \textit{posterior: }  q_{\phi}(\mathbf{z} | \mathbf{x}) = \softmax \left(-\frac{\| \hat{\mathbf{z}} - \mathcal{C} \|_2}{\tau}\right) \\
    & \textit{latent: } \mathbf{z} = q_{\phi}(\mathbf{z} | \mathbf{x}) \mathcal{C} \\ 
    & \textit{kl: } \mathcal{L}_{\mathrm{kl}} = H(q_{\phi}(\mathbf{z} | \mathbf{x}))- H\left(\mathbb{E}_{\mathbf{x} \sim p(\mathbf{x})} q_{\phi}(\mathbf{z} | \mathbf{x})\right) \\ 
\end{split}
$}
\end{equation}
where $\tau$ is the temperature parameter controlling the sharpness of the softmax probability and is set to $0.07$ by ablation. 
The derivation of $\mathcal{L}_{kl}$ is shown in \cref{sec:appendix-softvq-kl}.


Despite this simple modification, \softvq can significantly reduce the latent token length while maintaining a high quality of the reconstruction and latent space. 
More importantly, with a soft categorical distribution, \softvq is fully-differentiable, and thus the encoder and codebook can be optimized directly from the reconstruction loss (and other losses). 
% The conflicting codebook loss and commit loss used in \vq is no longer needed \cite{huh2023straightening}, and, in fact, we found that adding these loss terms hurts the latent space. 
It also allows for easier regularization of various forms on the latent space that drastically improves its quality, and less hyper-parameter tuning without codebook and commit loss \cite{huh2023straightening} in the reduced training objectives.


\noindent \textbf{Interpretation}. 
% \softvq also has good interpretability.
The posterior and latent space of \vq can be interpreted with K-Means \cite{lloyd1982least}.
Hence, \softvq can be viewed as soft K-Means \cite{dunn1973fuzzy}, with codewords as learnable prototypes in the latent space.
This latent space can easily be extended to Gaussian Mixture Models (GMM) \cite{reynolds2009gaussian}, which we refer to as \textbf{GMMVQ-VAE}.
Instead of using fixed temperature, GMMVQ-VAE predicts data-dependent weights for the codeword prototypes, \ie, Gaussian means, to compute the soft categorical posterior: $q_{\phi}(\mathbf{z}|\mathbf{x}) = \softmax(- \omega(\hat{\mathbf{z}})  \| \hat{\mathbf{z}} - \mathcal{C} \|_2 )$.
Although prior work has explored GMM-based VAEs \cite{dilokthanakul2016deep,johnson2016composing}, our GMMVQ-VAE differs by learning discrete prototypes rather than continuous latent variables.
% , enabling more structured representations.
While providing the additional benefit of interpretable Gaussian components in the latent space, GMMVQ achieves reconstruction quality and downstream generation performance similar to SoftVQ in our experiments, and thus we mainly adopt the simpler SoftVQ throughout this paper.
More details are in \cref{sec:appendix-softvq-gmm}.





\subsection{Representation Alignment of Latent Space}

While the reconstruction quality of tokenizer is important, learning a high-quality latent space is more crucial for downstream denoising-based generative modeling \cite{yu2024representation}.
Several recent approaches have explored aligning the latent code with pre-trained features through a contrastive loss \cite{ge2023plantingseedvisionlarge,wu2024vila,li2024imagefolder} and initializing the codebook with pre-trained features \cite{zhu2024scaling}. 
However, imposing effective regularization on the latent remains a challenge due to the discrete quantization of \vq and the Gaussian constraints in \kl. 

Thanks to the fully-differentiable property of \softvq, we can now directly impose regularization on the latent space.
Inspired by the recent work of REPA \cite{yu2024representation}, we propose aligning the representations of latent codes with pre-trained vision encoders to facilitate learning the latent space.
Compared to REPA, which aligns the representation at intermediate layers of downstream generative models, our method of feature alignment in the tokenizer's latent space is equivalent to performing REPA at the input space of generative models. 
Specifically, to align the latent code with the image tokens from a pre-trained vision encoder, we replicate each latent token by $N / L$ times:
\begin{equation}
    \mathbf{z}_r = [\underbrace{\mathbf{z}^{[0]}, \ldots, \mathbf{z}^{[0]}}_{N / L \text{ times}}, \underbrace{\mathbf{z}^{[1]}, \ldots, \mathbf{z}^{[1]}}_{N / L \text{ times}}, \ldots, \underbrace{\mathbf{z}^{[L]}, \ldots, \mathbf{z}^{[L]}}_{N / L \text{ times}}],
\end{equation}
and encourage the token-wise similarity with image tokens.
We employ a projector multilayer perceptron (MLP) on top of the latent tokens to match the pre-trained feature $\mathbf{y}_*$:
\begin{equation}
\mathcal{L}_{\mathrm{align}} = \frac{1}{N} \sum_{n=1}^N \operatorname{sim}\left(\mathbf{y}_*^{[n]}, \text{MLP}\left(\mathbf{z}_r^{([n]}\right)\right).
\end{equation}

This alignment ensures the latent space of \softvq captures semantically discriminative features that are beneficial for training the downstream generative models, even if it does not directly translate into improved reconstruction performance from the tokenizer. 
However, as we will show in \cref{sec:exp-latent}, the generation quality of trained generative models often depends more on the semantic structure of the latent space than on the tokenizer's reconstruction capabilities. 





\subsection{Final Training Objective}

The training objective of \softvq combines the reconstruction loss, perceptual loss \cite{larsen2016autoencoding,johnson2016perceptual,dosovitskiy2016generating,zhang2018unreasonableeffectivenessdeepfeatures} and adversarial loss \cite{goodfellow2020generative,isola2018imagetoimagetranslationconditionaladversarial} as in VQ \cite{esser2021taming}, and representation alignment:
\begin{equation}
\mathcal{L} = \mathcal{L}_{\textrm{recon}} + \lambda_1 \mathcal{L}_{\textrm{percep}} + \lambda_2 \mathcal{L}_{\textrm{adv}} + \lambda_3 \mathcal{L}_{\textrm{align}} + \lambda_4 \mathcal{L}_{\textrm{KL}},
\end{equation}
where $\lambda_1$, $\lambda_2$, $\lambda_3$, and $\lambda_4$ are hyper-parameters. 
Neither codebook nor commit loss as in VQ is needed.
The perceptual loss $\mathcal{L}_{\textrm{percep}}$ helps capture high-level perceptual features, $\mathcal{L}_{\textrm{adv}}$ encourages the decoder to generate realistic images by removing the artifacts from the reconstruction loss only, $\mathcal{L}_{\textrm{align}}$ guides the latent space to align with pre-trained features, and $\mathcal{L}_{\textrm{kl}}$ as the KL divergence term in the ELBO. 
% of \softvq.
% \wjd{Seems we have more hyperparameters to tune?}


\section{Experiments}
\label{sec:exp}

In this section, we validate the efficiency and effectiveness of \softvq with extensive experiments. 



\input{tables/main_256}

\subsection{Experiments Setup}
\label{sec:exp-setup}


\noindent \textbf{Implementation Details of \softvq}. 
We use the LlamaGen codebase \cite{sun2024autoregressive} to build our \softvq. 
We instantiate 4 configurations: SoftVQ-S, SoftVQ-B, SoftVQ-BL, SoftVQ-L, with a total of 45M, 173M, 391M, and 608M parameters, respectively.
% More details of the model configurations are shown in \cref{sec:appendix-exp-softvq}.
Each configuration has variants of latent codes $L=64$ and $L=32$.
For the representation alignment, we choose DINOv2 \cite{oquab2023dinov2} for the pre-trained features, similarly as \citet{yu2024representation} and \citet{li2024imagefolder}. 
To learn a better semantic latent space, we initialize our encoder from the pre-trained DINOv2 weights. 
Alignment with other pre-trained features is explored in \cref{sec:exp-latent}.
% Note that although we discussed several variants of SoftVQ, such as the combination with PQ \cite{jegou2010product}, RQ \cite{lee2022autoregressive}, and GMMVQ, they are only used in our ablation results. 
We train the tokenizers on ImageNet \cite{deng2009imagenet} of resolution 256$\times$256 and 512$\times$512 for 250K iterations. 
% AdamW \cite{loshchilov2017decoupled} optimizer is used with $\beta_1=0.9$, $\beta_2=0.95$, a weight decay of 1$e$-4, a maximum learning rate of 1$e$-4, and cosine annealing scheduler with a linear warmup of 5K steps.
% A constant batch size of 256 is used for all models.
Similarly to \citet{tian2024visualautoregressivemodelingscalable} and \citet{li2024imagefolder}, we found that the discriminator is very important for training tokenizer, and we adopted the same frozen DINO-S  \cite{caron2021emerging,oquab2023dinov2} discriminator with a similar architecture to StyleGAN \cite{karras2019style,karras2020analyzing}.
In addition, we use DiffAug \cite{zhao2020differentiable}, consistency regularization \cite{zhang2019consistency}, and LeCAM regularization \cite{tseng2021regularizinggenerativeadversarialnetworks} for discriminator training as in \cite{tian2024visualautoregressivemodelingscalable}.
For the training objective, we set $\lambda_1=1.0$, $\lambda_1=0.2$, $\lambda_3=0.1$, and $\lambda_4=0.01$, following previous common practice. 
More training details are shown in \cref{sec:appendix-exp-softvq}.


\noindent \textbf{Implementation Details of Generative Modeling}.
We select DiT \cite{peebles2023scalablediffusionmodelstransformers}, SiT \cite{li2024scalable}, and MAR \cite{li2024autoregressiveimagegenerationvector} for downstream denoising-based image generation tasks.
For DiT and SiT, we set the patch size of DiT and SiT to 1 and use a 1D absolution position embedding.
In our main experiments, we train DiT-XL and SiT-XL of 675M parameters for 3M steps, compared to 4M steps in REPA \cite{yu2024representation} and 7M steps vanilla version \cite{peebles2023scalablediffusionmodelstransformers,ma2024sit}.
We strictly follow their original training setup for other settings.
For MAR-H, we train for 500 epochs and set the maximum learning rate to 2$e$-4 since a higher learning rate leads to NAN issues.  
For other experiments, we simply train SiT-L of 458M parameters for 400K steps.
More experimental details are provided in \cref{sec:appendix-exp-gen}.




\noindent \textbf{Evaluation}.
We use reconstruction Frechet Inception Distance (rFID) \cite{heusel2017gans} on ImageNet validation set to evaluate the tokenizer.
To evaluate the performance of generation tasks, we report generation FID (gFID), Inception Score (IS) \cite{salimans2016improved}, Precision and Recall \cite{kynkaanniemi2019improved} (in \cref{sec:appendix-results-gen}), with and without classifier-free guidance (CFG) \cite{ho2022classifier}. 
We measure the efficiency of the generative models by GLOPs of the model's forward pass on the latent codes of tokenizers, and training and inference throughput for the models using floating point 32 and a batch size of $64$ on a single A100.



\subsection{Main Results}
\label{sec:exp-main}


We present the main reconstruction and generation results on the ImageNet benchmark of resolution 256$\times$256 and 512$\times$512 in \cref{tab:main_256} and \cref{tab:main_512}, respectively.
We show that \softvq achieves reconstruction and generation performance (with generative models) comparable to leading systems with 32 and 64 tokens, while presenting a significant improvement in both training and inference efficiency.

\noindent \textbf{Consistent high-quality reconstruction}.
% The reconstruction results demonstrate that 
SoftVQ variants achieve remarkable reconstruction quality with a high compression ratio.
With only 32 and 64 tokens, our models maintain consistent rFID scores, \ie, 0.61-0.89 on the 256$\times$256 and 0.64-0.71 on 512$\times$512 benchmark, substantially outperforming VQ tokenizers with 256 tokens used in autoregressive models such as MaskGIT \cite{chang2022maskgitmaskedgenerativeimage} and TiTok \cite{yu2024an}.
Our results are also comparable to KL tokenizers used in previous denoising-based models, using \textbf{32x} fewer tokens.  
More discussion of different tokenizers is given in \cref{sec:exp-compare}.

\input{tables/main_512}




\noindent \textbf{Generation performance comparable to SOTA}.
Notably, with only 32 tokens, the generation performance of DiT-XL and SiT-XL trained on all variants of the proposed SoftVQ significantly outperforms DiT-XL/2 and SiT-XL/2 with KL tokenizers of 1024 tokens, without using CFG. 
DiT-XL with SoftVQ-L of 32 tokens presents a \textbf{0.62} improvement on FID and SiT-XL with SoftVQ-L of 32 tokens shows a \textbf{0.71} improvement on FID,  without using CFG. 
The improvement is further strengthened with 64 tokens.
SiT-XL with SoftVQ-L of 64 tokens outperforms SiT-XL/2 with REPA \cite{yu2024representation}, without using CFG.
Applying CFG, SiT-XL with SoftVQ of 64 tokens achieves a performance comparable to the leading systems with the best FID as \textbf{1.78} on 256 and \textbf{2.21} on 512 benchmark.
Using MAR-H \cite{li2024autoregressiveimagegenerationvector}, SoftVQ-BL and SoftVQ-L with 64 and 32 tokens present slightly worse results, compared to the KL tokenizer of 256 tokens, possibly due to the lowered learning rate.
MAR-H and SiT-XL results on 512 benchmark with 32 tokens are included in \cref{sec:appendix-results-main}.



\noindent \textbf{Efficiency}.
The system-level comparison reveals SoftVQ's exceptional efficiency across multiple metrics. 
When integrated with MAR-H at 256$\times$256 resolution, SoftVQ reduces GFLOPs by ~\textbf{40}\% compared to standard KL tokenizer, \ie, 86.55 vs 145.08 GFLOPs with 64 tokens and further reducing to 67.93 GFLOPs with 32 tokens. 
The efficiency gains are even more pronounced in diffusion-based models, especially with higher resolutions.
SoftVQ enables DiT-XL and SiT-XL to achieve significantly lower computational costs \ie, 28.81 and 29.23 GFLOPs, respectively with 64 tokens, compared to their KL counterparts (80.73 GFLOPs with 1024 tokens).
Importantly, these efficiency improvements come without compromising generation quality.
SiT-XL trained on SoftVQ-BL with 64 tokens presents ~\textbf{55x} throughput than the KL counterpart, while showing competitive IS and FID scores in all configurations.
The improved GFLOPs also lead to a more efficient training. 
Not only do we require fewer training iterations to achieve a comparable performance to leading systems, \ie, 2.5M vs 7M steps of SiT-XL and DiT-XL, the high compression ratio of SoftVQ also improves the training throughput, reducing the time required to train SiT-XL for 400K steps from 72 to 20 hours on 8 A100.

% \ch{also mention training efficiency}








\subsection{Comparison of Tokenizers}
\label{sec:exp-compare}

We compare the proposed \softvq with the concurrent efficient image tokenizers, \ie, TiTok \cite{yu2024an} and DC-AE \cite{chen2024deep}. 
To show the superiority of \softvq in achieving a high compression ratio, we additionally train \vq and AE using the small (S) configuration and the same training recipe of SoftVQ. 
To validate the generation performance, we train a SiT-L for 400K steps and report gFID and IS on 256 ImageNet without using CFG, as shown in \cref{tab:tokenizer_compare}. 

\noindent \textbf{Scalable performance}.
With a much smaller model size, \ie, 46M vs 390M, SoftVQ-S significantly outperforms both TiTok variants at 64 tokens, achieving better reconstruction quality with an rFID of \textbf{1.03} compared to 1.25, and better generation performance with a gFID of \textbf{11.24} and IS of \textbf{89.4} compared to the best TiTok gFID of 19.23 and IS of 61.8. 
Noteworthy is that the generation results SiT-L trained on SoftVQ with 32 tokens outperform those trained on KL tokenizer with 1024 tokens \cite{ma2024sit} by a large margin, \ie, \textbf{5.9} in gFID.
Compared to DC-AE, SoftVQ-S demonstrates competitive scalability across token counts while maintaining significant generation quality even with fewer parameters.

\input{tables/tokenizer_compare}


\noindent \textbf{Less Lossy Property}.
SoftVQ-S exhibits remarkably consistent performance across different compression ratios. 
When reducing tokens from 256 to 32, SoftVQ-S maintains a minimal degradation in rFID from 0.80 to 1.24, significantly outperforming both VQ-S, from 1.45 to 10.97, and AE-S, from 1.15 to 2.01.
The benefits of the fully-differentiable property of SoftVQ along with representation alignment are particularly evident in generation quality, where SoftVQ-S achieves substantially better gFID of 9.21-12.89, and IS scores of 79.5-93.6, compared to baselines, showing its robustness in preserving information at high compression ratios and a better latent space for generative models to be trained on.





\subsection{Discussions on the Latent Space}
\label{sec:exp-latent}

We perform more analysis on the latent of SoftVQ here.
% showing that the proposed representation alignment in latent space results in not only superior generation performance but also better intermediate features of generative models.





\noindent \textbf{Alignment with different initialization and target models}.
As shown in \cref{tab:represent_align}, our results demonstrate the effectiveness of alignment across various pre-trained models. % \xl{maybe clarify codebook init. or encoder init.}
The encoder initialization and alignment with DINOv2-B \cite{oquab2023dinov2} achieve superior performance with rFID 0.88 and IS 103.4, compared to using either component alone.
Further improvements are observed with CLIP-B \cite{radford2021learning} and EVA-02-B \cite{fang2024eva} on reconstruction.
We reveal that a better rFID does not necessarily translate to a better gFID.
Instead, the latent space quality, reflected by linear probing accuracy, is more closely related to the performance of the generative models.
% , achieving generation performance of IS 109.3 and 112.7 and gFID scores of 9.89 and 10.34, respectively.





\noindent \textbf{Linear probing of tokenizer and generative model}.
Linear probing results in \cref{fig:linear_probing} (details in \cref{sec:appendix-exp-lp}) reveal SoftVQ's superior representation quality at both tokenizer and generative model. 
At the tokenizer level, the linear probing accuracy of SoftVQ variants (B, BL, L) consistently outperforms VQ-S and AE-S across all token counts, with the gaps widening at lower token counts, similarly observed by \citet{yu2024an}. 
This advantage transfers to the generative model with the best linear probing accuracy on the intermediate features of SiT trained with SoftVQ.
% outperforms the one trained with KL \cite{ma2024sit} using both 32 and 64 tokens and with REPA \cite{yu2024representation} using 32 tokens.
% accuracy (>55%) even with fewer tokens, significantly above the baseline SiT-XL performance.





\noindent \textbf{Latent space visualization}.
UMAP visualizations on the latent space in \cref{fig:latent_vis} demonstrate SoftVQ's ability to maintain structured and discriminative latent representations with minimal variance between encoder output ($\hat{\mathbf{z}}$) and decoder input ($\mathbf{z}$). 
% This stability persists even at high compression ratios (32 tokens), aligning with the superior linear probing results and generation performance.
Comparing \cref{fig:latent_vis} (d) and (c), we also observe the larger encoder can learn a more discriminative latent space, showing the superiority of SoftVQ's representation learning.

% \xl{maybe add one sentence to explain why (d) is different from (b)(c) even though due to systematic issue}



\subsection{Ablation Studies}
\label{sec:exp-ablation}


We present a series of ablation studies in \cref{sec:appendix-results-ablation}, including SoftVQ variants with product quantization (PQ) \cite{jegou2010product}, residual quantization (RQ) \cite{lee2022autoregressive}, and GMMVQ, codebook size, latent space size, and the temperature of SoftVQ.
The results show the compatibility of SoftVQ with PQ and RQ, with slightly improved performance.
GMMVQ presents results comparable to SoftVQ.
Moreover, SoftVQ shows robustness to other parameters, such as codebook size and softmax temperature. 
We found that while increasing the dimension of the latent space can result in a significant improvement in reconstruction, it leads to deterioration in generation performance, possibly due to the learning difficulty of generative models with larger dimensions \cite{sohl2015deep}.

\input{tables/represent_align}




\section{Related Work}
\label{sec:related}

\noindent \textbf{Image tokenization} has emerged as a fundamental technique to bridge various vision tasks. Traditional approaches using autoencoders \cite{hinton2006reducing,vincent2008extracting} laid the groundwork by compressing images into latent representations. This field subsequently diverged into two main branches: generation-focused and understanding-focused approaches. Generation-oriented methods, such as VAE \cite{van2017neural,razavi2019generating} and VQ-GAN \cite{esser2021taming,razavi2019generatingdiversehighfidelityimages}, emphasized learning latent spaces for detail-preserving compression. These were further refined through variants \cite{lee2022autoregressive,yu2023language,mentzer2023finite,zhu2024scaling} that enhanced generation quality. Parallel developments in understanding-focused approaches leveraged Large Language Models (LLMs) \cite{vaswani2023attentionneed} to create semantic representations for tasks like classification \cite{dosovitskiy2021imageworth16x16words} and detection \cite{zhu2010deformable}. Recent work \cite{yu2024an,li2024imagefolder} has demonstrated the potential of unifying these approaches, with subsequent research \cite{wu2024vila,gu2023rethinkingobjectivesvectorquantizedtokenizers} exploring the convergence of generation and understanding capabilities using a single tokenizer.

% \paragraph{Image generation}
\noindent \textbf{Image generation} have two popular paradigms: autoregressive and diffusion. 
% Autoregressive and diffusion are two popular image generation paradigms. 
Autoregressive models start from CNN-based architectures \cite{van2016conditional} and evolve to the transformer-based architectures \cite{vaswani2023attentionneed,yu2024randomized,lee2022autoregressive,liu2024customize,sun2024autoregressive} to enhance scalability. Latest works in visual autoregressive modeling, including VAR \cite{tian2024visualautoregressivemodelingscalable}, MAR \cite{li2024autoregressiveimagegenerationvector}, and ImageFolder \cite{li2024imagefolder}, have further enhanced generation efficiency. 
Diffusion models have transformed image generation since their introduction by Sohl-Dickstein et al. \cite{sohldickstein2015deepunsupervisedlearningusing}. Key advancements by Nichol et al. \cite{nichol2021improveddenoisingdiffusionprobabilistic}, Dhariwal et al. \cite{dhariwal2021diffusionmodelsbeatgans}, and Song et al. \cite{song2022denoisingdiffusionimplicitmodels} have significantly improved model performance. A paradigm shift occurred with the adoption of latent space diffusion \cite{vahdat2021scorebasedgenerativemodelinglatent,rombach2022highresolutionimagesynthesislatent}, leveraging pre-trained image encoders as priors \cite{van2017neural,esser2021taming} to enhance generation efficiency. Architectural innovations, particularly the integration of transformers \cite{peebles2023scalablediffusionmodelstransformers}, have further expanded the capabilities of these models.
These advances have spawned numerous influential systems, from text-guided generation \cite{nichol2021glide,ding2021cogview} to high-fidelity synthesis \cite{gafni2022make,saharia2022photorealistic}. 
Commercial successes \cite{ramesh2021zero,rombach2022high,midjourney,sora} have also demonstrated the practical impact of diffusion models.


\begin{figure}[t!]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/linear_probing.pdf}
    \vspace{-0.15in}
    \caption{Linear probing accuracy of ImageNet-1K val. set on (a) latent tokens of tokenizer and (b) intermediate features (layer 20) of SiT (L for small and XL for others) trained on latents of tokenizer.}
    \label{fig:linear_probing}
\vspace{-0.15in}
\end{figure}



\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/latent.pdf}
    \vspace{-0.1in}
    \caption{Visualization of $\hat{\mathbf{z}}$ (top), \ie, encoder output, and $\mathbf{z}$ (bottom), \ie, decoder input, of (a) VQ-S 64; (b) SoftVQ-S 64; (c) SoftVQ-S 32; (d) SoftVQ-L 32, trained with latent space alignment.
    %SoftVQ presents significantly more discriminative latent representations with less variance loss between $\hat{\mathbf{z}}$ and $\mathbf{z}$, which transfers to the better performance of generative models.
    }
    \label{fig:latent_vis}
\vspace{-0.2in}
\end{figure}


\section{Conclusion}
\label{sec:conclusion}
We presented \softvq, a continuous image tokenizer leveraging soft categorical posteriors to aggregate multiple codewords into each latent token. 
Our approach compresses images to just 32 or 64 tokens while maintaining high reconstruction quality and enabling state-of-the-art generation results with DiT, SiT, and MAR. The substantial improvements in both inference throughput (up to 55x with 64 tokens) and training efficiency, combined with the fully-differentiable design's ability to learn semantic-rich representations, demonstrate \softvq's potential as a foundation for efficient generative and vision-language models.




==> tables/main_full_256_old.tex <==
\begin{table*}[]
\centering
\caption{\ch{Ugly}}
\label{tab:my-table}
\resizebox{0.95 \textwidth}{!}{%
\begin{tabular}{@{}lc|lccc|ccc|cc|cc@{}}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Gen. \\ Model\end{tabular}}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Gen.\\ \# Params\end{tabular}} &
  \multirow{2}{*}{Tokenizer} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Tokenizer\\ \# Params\end{tabular}} &
  \multirow{2}{*}{\# Tokens} &
  \multirow{2}{*}{rFID} &
  \multirow{2}{*}{Gflops} &
  \multirow{2}{*}{Steps} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Throughput\\ (imgs/sec.)\end{tabular}} &
  \multicolumn{2}{c|}{\small{w/o CFG}} &
  \multicolumn{2}{c}{\small{w/ CFG}} \\
\multicolumn{1}{c}{} &
   &
   &
   &
   &
   &
   &
   &
   &
  gFID &
  IS &
  gFID &
  IS \\ \midrule

\multicolumn{13}{c}{\textbf{Diffusion-based}} \\ \toprule

  
LDM-4 \cite{rombach2022high} &
  400M &
  KL-4 \cite{rombach2022high} &
    &
  4096$\times$3 &
  0.27 &
   &
  250 &
  0.40 &
  10.56 &
  103.5 &
  3.60 &
  247.7 \\  \midrule
DiffiT \cite{hatamizadeh2025diffit} &
  - &
  KL &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
  1.73 &
  276.5 \\ \midrule
U-ViT-H/2 \cite{bao2023all} &
  501M &
  \multirow{7}{*}{KL-8 \cite{stabilityai2023}} &
  \multirow{7}{*}{} &
  \multirow{7}{*}{1024$\times$4} &
  \multirow{7}{*}{0.62} &
  128.89 &
  50 &
  1.01 &
  - &
  - &
  2.29 &
  263.9 \\ \cmidrule(r){1-2} \cmidrule(l){7-13} 
MDTv2-XL/2 \cite{gao2023mdtv2} &
  676M &
   &
   &
   &
   &
   125.43 &
   250 &
   0.62 &
  5.06 &
  155.6 &
  1.58 &
  314.7 \\ \cmidrule(r){1-2} \cmidrule(l){7-13} 
DiT-XL/2 \cite{li2024scalable} &
  \multirow{2}{*}{675M} &
   &
   &
   &
   &
  \multirow{2}{*}{80.73} &
  \multirow{2}{*}{250} &
  \multirow{2}{*}{0.53} &
  9.62 &
  121.5 &
  2.27 &
  278.2 \\
+ REPA \cite{yu2024representation} &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\ \cmidrule(r){1-2} \cmidrule(l){7-13} 
SiT-XL/2 \cite{ma2024sit} &
  \multirow{3}{*}{675M} &
   &
   &
   &
   &
  \multirow{3}{*}{80.73} &
  \multirow{3}{*}{250} &
  \multirow{3}{*}{0.57} &
  8.30 &
  131.7 &
  2.06 &
  270.3 \\
+ REPA \cite{yu2024representation} &
   &
   &
   &
   &
   &
   &
   &
   &
  5.90 &
  157.8 &
  1.80 &
  284.0 \\
+ REPA * &
   &
   &
   &
   &
   &
   &
   &
   &
  5.90 &
  157.8 &
  1.42 &
  305.7 \\ \midrule
\multirow{6}{*}{DiT-XL} &
  \multirow{6}{*}{675M} &
  \multirow{2}{*}{SoftVQ-B} &
  \multirow{2}{*}{173M} &
  64 &
  0.88 &
  28.81 &
  250 &
  4.81 &
   &
   &
   &
   \\
 &
   &
   &
     &
  32 &
  0.89 &
  14.52 &
  250 &
  9.12 &
   &
   &
   &
   \\ \cmidrule(l){3-13} 
 &
   &
  \multirow{2}{*}{SoftVQ-BL} &
  \multirow{2}{*}{391M} &
  64 &
  0.65 &
  28.81 &
  250 &
  4.69 &
   &
   &
   &
   \\
 &
   &
   &
   &
  32 &
  0.68 &
  14.52 &
  250 &
  8.92 &
   &
   &
   &
   \\ \cmidrule(l){3-13} 
 &
   &
  \multirow{2}{*}{SoftVQ-L} &
  \multirow{2}{*}{608M} &
  64 &
  0.61 &
  28.81 &
  250 &
  4.59 &
   &
   &
   &
   \\
 &
   &
   &
   &
  32 &
  0.74 &
  14.52 &
  250 &
  8.84 &
   &
   &
   &
   \\ \midrule
\multirow{6}{*}{SiT-XL} &
  \multirow{6}{*}{675M} &
  \multirow{2}{*}{SoftVQ-B} &
  \multirow{2}{*}{173M} &
  64 &
  0.88 &
  29.23 &
  250 &
  5.60 &
   &
   &
   &
   \\
 &
   &
   &
   &
  32 &
  0.89 &
  14.73 &
  250 &
  10.36 &
   &
   &
   &
   \\ \cmidrule(l){7-13} 
 &
   &
  \multirow{2}{*}{SoftVQ-BL} &
  \multirow{2}{*}{391M} &
  64 &
  0.65 &
  29.23 &
  250 &
  5.51 &
   &
   &
   &
   \\
 &
   &
   &
   &
  32 &
  0.68 &
  14.73 &
  250 &
  10.22 &
   &
   &
   &
   \\ \cmidrule(l){7-13} 
 &
   &
  \multirow{2}{*}{SoftVQ-L} &
  \multirow{2}{*}{608M} &
  64 &
  0.61 &
 29.23  &
  250 &
  5.49 &
   &
   &
   &
   \\
 &
   &
   &
   &
  32 &
  0.74 &
  14.73 &
  250 &
  10.19 &
   &
   &
   &
   \\ \bottomrule
\multicolumn{13}{c}{\textbf{AR-based}} \\ \toprule

Taming-Trans. \cite{esser2021taming} &
  \multirow{2}{*}{1.4B} &
  \multirow{2}{*}{VQ \cite{esser2021taming}} &
  \multirow{2}{*}{-} &
  \multirow{2}{*}{256} &
  \multirow{2}{*}{7.94} &
  \multirow{2}{*}{-} &
  \multirow{2}{*}{-} &
   \multirow{2}{*}{-} &
  15.78 &
  78.3 &
  - &
  - \\
+ re.  &
   &
   &
   &
   &
   &
   &
   &
   &
  5.20 &
  290.3 &
  - &
  - \\ \midrule
RQ-Trans. \cite{lee2022autoregressive} &
  \multirow{2}{*}{3.8B} &
  \multirow{2}{*}{RQ \cite{lee2022autoregressive}} &
  \multirow{2}{*}{104M} &
  \multirow{2}{*}{256} &
  \multirow{2}{*}{3.20} &
  \multirow{2}{*}{908.81}  &
  \multirow{2}{*}{64} &
  \multirow{2}{*}{8.95} &
  7.55  &
  134.0 &
  - &
  - \\
+ re. &
   &
   &
   &
   &
  &
   &
  &
   &
  3.80 &
  323.7 &
  - &
  - \\ \midrule
MaskGIT \cite{chang2022maskgitmaskedgenerativeimage} &
  227M &
  VQ \cite{chang2022maskgitmaskedgenerativeimage} &
   &
  256 &
  2.28 &
   &
   &
   &
  6.18 &
  182.1 &
  - &
  - \\ \midrule
MAGE \cite{li2023magemaskedgenerativeencoder} &
  230M &
  VQ \cite{esser2021taming} &
   &
   &
   &
   &
   &
   &
  6.93 &
  195.8 &
  - &
  - \\ \midrule
VAR \cite{tian2024visualautoregressivemodelingscalable} &
  2.0B &
  MS-VQ \cite{tian2024visualautoregressivemodelingscalable} &
  109M &
  680 &
  0.90 &
 683.67 &
  10 &
  24.87 &
  - &
  - &
  1.92 &
  323.1 \\ \midrule
ImageFolder \cite{li2024imagefolder} &
  362M &
  MS-VQ \cite{li2024imagefolder} &
  178M &
  265 &
  0.80 &
  - &
  10 &
  - &
  - &
  - &
  2.60 &
  295.0 \\ \midrule
LlamaGen \cite{sun2024autoregressive} &
  3.1B &
  VQ \cite{sun2024autoregressive} &
  72M &
  256 &
  2.19 &
  781.56 &
  256 &
  3.20 &
  - &
  - &
  3.06 &
  279.71 \\ \midrule
TiTok-S-128 \cite{yu2024an} &
  287M &
  VQ  \cite{yu2024an} &
  72M &
  128 &
  1.71 &
  33.03 &
  64 &
  6.71 &
  - &
  - &
  1.97 &
  281.8 \\ \midrule
MaskBit \cite{weber2024maskbit} &
  305M &
  LFQ \cite{weber2024maskbit} &
  54M &
  256 &
  1.61 &
  - &
  256 &
  - &
  - &
  - &
  1.52 &
  328.6 \\ \midrule
MAGViT-v2 \cite{yu2023language} &
  307M &
  LFQ \cite{yu2023language} &
  116M &
  256 &
  1.61 &
  - &
  64 &
  - &
  - &
  - &
  1.78 &
  319.4 \\ \midrule
% OpenMAGVIT-v2 \cite{luo2024open} &
%   1.5B &
%   LFQ \cite{luo2024open} &
%   115M &
%   256 &
%   1.17 &
%    &
%   256 &
%    &
%   - &
%   - &
%   2.33 &
%   271.7 \\ \midrule
MAR-H \cite{li2024autoregressiveimagegenerationvector} &
  945M &
  KL &
   &
  256 &
   &
   145.08 &
   256 &
  0.01 &
  2.35 &
  227.8 &
  1.55 &
  303.7 \\ 
 \bottomrule
 
\end{tabular}%
}
\end{table*}
